Preemptively Pruning Clever-Hans Strategies in Deep Neural Networks

Robustness has become an important consideration in deep learning. With the help of explainable AI, mismatches between an explained model's decision strategy and the user's domain knowledge (e.g. Clever Hans effects) have been identified as a starting point for improving faulty models. However, it is less clear what to do when the user and the explanation agree. In this paper, we demonstrate that acceptance of explanations by the user is not a guarantee for a machine learning model to be robust against Clever Hans effects, which may remain undetected. Such hidden flaws of the model can nevertheless be mitigated, and we demonstrate this by contributing a new method, Explanation-Guided Exposure Minimization (EGEM), that preemptively prunes variations in the ML model that have not been the subject of positive explanation feedback. Experiments demonstrate that our approach leads to models that strongly reduce their reliance on hidden Clever Hans strategies, and consequently achieve higher accuracy on new data.

==> bu1.tex <==
%placeholder

==> bu2.tex <==
%placeholder

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

# This block is for the purpose of first generating the aux files, and then compiling the main file again (for bibunits: https://www.overleaf.com/learn/latex/Questions/Creating_multiple_bibliographies_in_the_same_document)
# Run BibTeX on all .aux files
$cleanup_includes_cusdep_generated = 1;
add_cus_dep('aux', 'bbl', 0, 'run_bibtex');
sub run_bibtex {
    my $file = $_[0];
    return system("bibtex '$file'");
}
$pdflatex = 'pdflatex -interaction=nonstopmode %O %S';
$pdflatex_silent = 'pdflatex -interaction=batchmode %O %S';
$pdf_mode = 1;
@generated_exts = (@generated_exts, 'blg', 'run_bibtex');
